Are Elites Meritocratic and Efficiency-Seeking? Evidence from MBA Students

Elites disproportionately influence policymaking, yet little is known about their fairness and efficiency preferences -- key determinants of support for redistributive policies. We investigate these preferences in an incentivized lab experiment with future elites: Ivy League MBA students. We find that MBA students implement substantially more unequal earnings distributions than the average American, regardless of whether inequality stems from luck or merit. Their redistributive choices are also far more responsive to efficiency costs than the near-zero response found in representative U.S. samples. These patterns partly reflect distinct fairness ideals: a large share of MBA students falls outside standard classifications, instead displaying "weak meritocratic" tendencies that tolerate inequality even when it stems from luck. These findings identify a channel through which elite preferences may sustain U.S. inequality.

==> results/corr_ideals_N.tex <==
Mean Dep. Var.&&0.181&&0.188&&0.277&&0.063&&0.292&\\
N (Spectators)&&271&&271&&271&&271&&271&\\


==> results/corr_ideals_age_over28.tex <==
Aged 28 or over&&0.016&&0.031&&0.029&&$-$0.016&&$-$0.060&\\
&&(0.045&)&(0.050&)&(0.057&)&(0.032&)&(0.058&)\\


==> results/corr_ideals_bonf_gini.tex <==
Implemented inequality&&0.489&\sym{***}&$-$0.050&&$-$0.330&\sym{***}&$-$0.207&\sym{***}&0.099&\\
&&(0.060&)&(0.048&)&(0.073&)&(0.051&)&(0.065&)\\


==> results/corr_ideals_born_usa.tex <==
Born USA&&0.064&&$-$0.027&&$-$0.026&&0.007&&$-$0.019&\\
&&(0.044&)&(0.051&)&(0.058&)&(0.031&)&(0.058&)\\


==> results/corr_ideals_comfortable.tex <==
Always enough money&&0.030&&0.055&&$-$0.015&&$-$0.009&&$-$0.062&\\
&&(0.045&)&(0.050&)&(0.058&)&(0.032&)&(0.060&)\\


==> results/corr_ideals_entrep.tex <==
Wants entrepreneur&&0.049&&$-$0.020&&$-$0.029&&0.044&&$-$0.044&\\
&&(0.046&)&(0.049&)&(0.057&)&(0.032&)&(0.058&)\\


==> results/corr_ideals_gini.tex <==
Implemented inequality&&0.489&\sym{***}&$-$0.050&&$-$0.330&\sym{***}&$-$0.207&\sym{***}&0.099&\\
&&(0.060&)&(0.048&)&(0.073&)&(0.051&)&(0.065&)\\


==> results/corr_ideals_hard_work.tex <==
Hard work better life&&0.032&&0.075&&$-$0.034&&0.030&&$-$0.103&\\
&&(0.055&)&(0.056&)&(0.075&)&(0.035&)&(0.078&)\\


==> results/corr_ideals_long_hours.tex <==
Long hours necessary&&$-$0.042&&0.130&\sym{***}&$-$0.103&&0.031&&$-$0.016&\\
&&(0.062&)&(0.049&)&(0.077&)&(0.034&)&(0.074&)\\


==> results/corr_ideals_luck_connect.tex <==
Success luck network&&0.015&&$-$0.109&\sym{**}&$-$0.048&&0.065&\sym{*}&0.076&\\
&&(0.048&)&(0.047&)&(0.059&)&(0.036&)&(0.061&)\\


==> results/corr_ideals_male.tex <==
Male&&0.146&\sym{***}&$-$0.082&&$-$0.102&\sym{*}&$-$0.038&&0.075&\\
&&(0.042&)&(0.050&)&(0.057&)&(0.032&)&(0.057&)\\


==> results/corr_ideals_manag.tex <==
Wants manager&&0.019&&0.008&&$-$0.079&&$-$0.026&&0.079&\\
&&(0.077&)&(0.087&)&(0.107&)&(0.064&)&(0.095&)\\


==> results/corr_ideals_nonprofit.tex <==
Career in a non$-$profit&&$-$0.021&&0.019&&$-$0.023&&0.056&&$-$0.032&\\
&&(0.058&)&(0.067&)&(0.074&)&(0.051&)&(0.075&)\\


==> results/corr_ideals_private_sec.tex <==
Career in priv. sector&&0.067&&$-$0.095&&0.086&&$-$0.037&&$-$0.021&\\
&&(0.053&)&(0.074&)&(0.072&)&(0.049&)&(0.079&)\\


==> results/corr_ideals_stay_usa.tex <==
Stay USA&&0.080&&0.002&&$-$0.260&\sym{*}&0.001&&0.178&\sym{*}\\
&&(0.069&)&(0.107&)&(0.133&)&(0.067&)&(0.093&)\\


==> results/corr_ideals_voted_last_elections.tex <==
Voted last elections&&0.007&&$-$0.044&&0.159&\sym{***}&0.041&&$-$0.163&\sym{**}\\
&&(0.048&)&(0.057&)&(0.056&)&(0.030&)&(0.065&)\\


==> results/corr_ideals_worklife_bal.tex <==
Work$-$life balance&&$-$0.038&&0.093&\sym{*}&$-$0.043&&0.033&&$-$0.044&\\
&&(0.046&)&(0.049&)&(0.057&)&(0.031&)&(0.058&)\\


==> results/gini_order_Nd.tex <==
\(N\) (decisions)&&261&&263&&269&&793&\\


==> results/ideals_almas_nor_all.tex <==
\cite{almas.etal2020} -- Average Norwegian &13.81 &42.45 &35.63 &8.11 \\
 &(1.89) &(3.46) &(2.62) &(4.74) \\


==> results/ideals_almas_nor_below100k.tex <==
\cite{almas.etal2020} -- NOR income below 100k &14.83 &42.68 &34.88 &7.62 \\
 &(2.09) &(3.75) &(2.85) &(5.15) \\


==> results/ideals_almas_nor_over100k.tex <==
\cite{almas.etal2020} -- NOR income over 100k &6.98 &41.77 &39.62 &11.63 \\
 &(3.93) &(9.06) &(6.78) &(11.98) \\


==> results/ideals_average.tex <==
Unweighted Average &22.67 &44.94 &13.99 &18.40 \\
 &(1.55) &(2.05) &(1.06) &(2.78) \\
Inverse-variance Weighted &12.67 &46.72 &14.59 &22.90 \\
 &(0.84) &(1.59) &(0.92) &(2.06) \\
Random Effects \citep{dersimonian1986meta} &21.81 &45.45 &14.37 &18.95 \\
 &(5.60) &(5.26) &(1.47) &(6.05) \\


==> results/ideals_dyson_usa.tex <==
Dyson students &23.91 &37.60 &1.85 &36.63 \\
 &(6.36) &(7.78) &(1.85) &(10.22) \\


==> results/ideals_hs_between.tex <==
\cite{harrs2023fairness} (spectators' first choices) &8.68 &45.24 &14.61 &31.46 \\
 &(1.04) &(2.30) &(1.30) &(2.84) \\


==> results/ideals_hs_within.tex <==
\cite{harrs2023fairness} (repeated-measures design) &5.42 &48.58 &10.77 &35.23 \\
 &(0.59) &(1.30) &(0.81) &(1.64) \\


==> results/ideals_mba_usa.tex <==
MBA students &23.16 &22.65 &9.89 &44.30 \\
 &(4.35) &(5.99) &(3.15) &(8.05) \\


==> results/ideals_sce_between.tex <==
SCE (spectators' first choices) &39.77 &36.67 &8.57 &14.99 \\
 &(5.25) &(6.31) &(2.75) &(8.66) \\


==> results/ideals_sce_within.tex <==
SCE (repeated-measures design) &26.40 &40.61 &4.57 &28.43 \\
 &(2.22) &(2.48) &(1.05) &(3.49) \\


==> results/narrative.tex <==
Libertarian&&0.133&&0.067&&0.067&&0.133&&0.067&&0.133&\\
&&(0.090&)&(0.066&)&(0.066&)&(0.090&)&(0.066&)&(0.090&)\\
Moderate&&0.222&&0.148&&0.185&&0.037&&0.148&&0.148&\\
&&(0.082&)&(0.070&)&(0.077&)&(0.037&)&(0.070&)&(0.070&)\\
Meritocrat&&0.361&&0.083&&0.111&&0.083&&0.167&&0.139&\\
&&(0.082&)&(0.047&)&(0.054&)&(0.047&)&(0.064&)&(0.059&)\\
Egalitarian&&0.250&&0.125&&0.125&&0.000&&0.000&&0.250&\\
&&(0.157&)&(0.120&)&(0.120&)&&&&&(0.157&)\\


==> results/narrative_N.tex <==
\(N\) (individuals)&&86&&86&&86&&86&&86&&86&\\


==> results/summ_dem.tex <==
Age $\le$23 &0.031 &0.174 &258 \\
Age 24--27 &0.380 &0.486 &258 \\
Age 28--31 &0.453 &0.499 &258 \\
Age $\ge$32 &0.136 &0.343 &258 \\
Male &0.554 &0.498 &260 \\
Cohort 2023 &0.509 &0.501 &271 \\
Cohort 2024 &0.491 &0.501 &271 \\
Born in the USA &0.562 &0.497 &256 \\


==> results/summ_emp.tex <==
Planning on getting a job in the USA &0.941 &0.237 &253 \\
Working long hours is sometimes necessary &0.811 &0.392 &254 \\
Wants career in a non-profit &0.173 &0.379 &254 \\
Wants to become an entrepreneur &0.484 &0.501 &254 \\
Wants career in private sector &0.839 &0.369 &254 \\
Work-life balance is more important than a high salary &0.524 &0.500 &254 \\
Aspire to be a manager &0.913 &0.282 &254 \\


==> results/summ_inc.tex <==
Always had enough money for necessities and luxuries &0.198 &0.399 &258 \\
Always had enough for necessities and occasional luxuries &0.422 &0.495 &258 \\
Usually had enough for necessities, rarely for luxuries &0.279 &0.449 &258 \\
Sometimes did not have enough money for necessities &0.081 &0.274 &258 \\
Frequently did not have enough money for necessities &0.019 &0.138 &258 \\


==> results/summ_pol.tex <==
Voted in the last elections &0.693 &0.462 &251 \\
Success is luck and connections &0.362 &0.482 &254 \\
Hard work brings a better life &0.815 &0.389 &254 \\


==> results/summ_qua.tex <==
Completed all three redistributive decisions &0.959 &0.198 &271 \\
Passed attention check &0.933 &0.250 &254 \\
Minutes spent in survey &4.553 &1.398 &271 \\

